MoPE: Mixture of Prefix Experts for Zero-Shot Dialogue State Tracking

Zero-shot dialogue state tracking (DST) transfers knowledge to unseen domains, reducing the cost of annotating new datasets. Previous zero-shot DST models mainly suffer from domain transferring and partial prediction problems. To address these challenges, we propose Mixture of Prefix Experts (MoPE) to establish connections between similar slots in different domains, which strengthens the model transfer performance in unseen domains. Empirical results demonstrate that MoPE-DST achieves the joint goal accuracy of 57.13% on MultiWOZ2.1 and 55.40% on SGD.

==> chapter/analysis.tex <==
\subsection{Analysis on DPPT}

\input{table/random-prompt.tex}

\input{table/ICL.tex}

\paragraph{Comparasion between DPPT and ICL}

To better investigate the initial ability of the LLM and the effect of deep prefix prompt tuning (DPPT) for LLM, we compare the results of in-context learning (ICL) and DPPT. We evaluate the performance of ICL and the performance of DPPT with less training data about 5\% of the whole training data. The experimental results shown in table~\ref{table: ICL}, we find that LLM hardly solves the DST problem well with the initial frozen pre-trained model although we have fed up to 5 examples for the LLM to simulate. Compared to the frozen LLM, adding a well-trained deep prefix prompt to the frozen model significantly improves the performance. This means that the pre-trained LLM isn't trained well on DST datasets but we can add a well-trained deep prefix prompt to improve the ability of LLM on DST.

\subsection{Analysis on MPPE}

\paragraph{Analysis on the specificity of prefix prompt}

To investigate the specificity of prefix prompt, we conduct experiments on the performance of random prefix prompt and specialized prefix prompt, the result is shown in table~\ref{table: random-prompt}. The result shows random prefix prompt will cause a sharp drop in performance, which means well trained prefix prompt is specialized for specific slots and not suitable for all slots.


\paragraph{Analysis on the feature of clustering}

\input{fig/cluster-example.tex}

\input{fig/compare-feature.tex}

The representation of the slot feature directly influences the dividing of clusters and has a huge impact on the final result. To study the effect of different feature representations of clustering on dialogue state tracking, We try two ways to represent the feature of the slots: the word embedding and the model hidden output. The experimental results are shown in Fig~\ref{fig:compare-feature}, we compare the results of different clustering features in the attraction domain under zero-shot experiments. We find that using hidden output as the clustering feature is significantly better than using the word embedding feature apart from the number of clusters being 1. To investigate the reason for this, we visualize the clustering result of the hidden output and the word embedding in Fig~\ref{fig: cluster example}. We believe that clustering by hidden output can gather more similar slots, so we use the hidden output as the clustering feature in the other experiments.

\paragraph{Analysis on the number of clusters}

\input{fig/num-clusters.tex}
\input{fig/heatmap.tex}

To study the impact of the number of clusters on the result,  We conduct experiments to investigate the influence of the number of clusters. We compare the results of different numbers of clusters in five zero-shot domains, the results are shown in Fig~\ref{fig: number-cluster}. As the number of clusters increases, the results climb up and then decline. In three of five domains, the best results are approached when the number of clusters is 2. For the other two domains, the best results are approached when the number of clusters is 1 and 3. We suspect the reason for the difference in the best cluster number is due to the different distribution of training slots, but the result is still sufficient to show that MPPE outperforms DPPT in most instances.

\paragraph{Analysis on the similarity of slots}

\input{table/cosine-similarity.tex}

To investigate the reason for the improvement of the MPPE,  We visualize the cosine similarity(ACS) matrix for all slot features on the restaurant domain experiment in Fig~\ref{fig: heatmap}. We can see that the similarity between different slots varies greatly. Our motivation for MPPE is to divide these slots into different clusters and maximize the similarity of slots in the same clusters to improve the performance of predicting slots. We calculate the average cosine similarity for both train and test slots in Table~\ref{table: ACS}. We find that higher average cosine similarity tends to show better performance, which means that more similar and relevant slots in each cluster can improve the overall performance. We also find higher ACS of train slots doesn't ensure higher performance but higher ACS of test slots always shows better performance.

\input{fig/error-rate.tex}

\subsection{Error Analysis}

To investigate the reason for the improvement of MPPE, we analyze the slot error distribution of MPPE and DPPT in fig~\ref{fig: error-rate}. We divide slot errors into three categories: partial-prediction, over-prediction, and other errors. ``partial-prediction'' and ``over-prediction'' indicate model predicts less or more dialogue states respectively. We find that MPPE has less slot error, especially in ``partial-prediction''. We suspect that because specialized prompt makes LLM more sensitive to the relevant contents in the dialogue, which results in less ``partial-prediction'' and more ``over-prediction''. However, the decrease in total slot errors leads to an overall improvement in performance.



==> chapter/introduction-back.tex <==
\section{Introduction}

% zhutong: 第一段逻辑，每行一到两句话：任务定义和问题背景
%   先介绍一下 zero-shot DST 任务的目标是啥，是为了干啥，加参考文献
%   考虑把 Figure 1 改成 zero-shot DST，讲下 zero-shot DST 的流程。另外，Figure 1 的字有点小了，考虑加大一点，可以只用两个case
%   zero-shot DST 存在的问题和挑战：（1）如何利用已知领域的知识；（2）生成式方案存在over/partial prediction的问题。要加参考文献

% zhutong：第二段逻辑：现有方案和现存问题。每个点两句话左右，要加参考文献
%   针对已知领域的迁移，其他人是怎么做的，他们有什么问题没有解决
%   针对生成式DST，其他人是怎么做的，他们还有什么问题没有解决

Dialogue state tracking (DST) plays an important role in task-oriented dialogue (TOD) systems.
The goal of this task is to understand the user's needs and intentions from the dialogue, which helps the TOD system give responses that are more in line with the user's preferences and needs.

As we all know collecting and annotating DST data is hard and expensive, but the current DST models need a lot of relevant supervised data to perform well. It is still difficult for an existing DST model to perform well when directly transferring to a new domain. Therefore it is important and meaningful to research adapting the existing DST model to a new domain without supervised data. Apart from the challenge in domain adaption, DST models also have difficulty extracting the correct value of the corresponding slot for the diversity of the dialogue topics and the infinite possibility of the dialogue contents. It always gives wrong values, i.e. over-prediction and partial prediction \citep{xie-etal-2022-correctable}, which makes the TOD system have difficulty precisely understanding the intention of the user.

\input{fig/dialogue.tex}

% zhutong：第三段：我们的方法
%   针对上述zero-shot中的知识迁移问题，我们将多个领域的DST任务进行分解，并将新领域的任务归纳为某一个已经学习的领域中（注：这里我说的“领域”不太不准确，不是DST中的domain）
%   我们使用多个特异性专家(specialized experts)学习domain-slot知识
%   我们利用无监督聚类的方法，将domain-slot知识分成多个簇，并针对每个簇训练一个单独的专家
%   在zero-shot推理时，我们使用上述的无监督聚类方法进行路由分发，并使用已知领域专家解决新领域的DST任务
%   针对上述挑战中的第二个问题，我们使用LLM来减轻生成的错误
%   为了减少LLM的训练代价，我们使用PEFT方法进行训练，每个专家使用不同的prefix prompt表示

Mixture-of-experts (MoE) models do well in solving different kinds of tasks with the related expert model. There is a huge difference between different domains and slots in DST, such as ``hotel parking'' and ``hotel name'', it's an ideal way to take the way of MoE to deal with this. We can split the whole DST task into several subtasks based on the domain and slot and try to use the MoE model to solve each subtask. \citet{wang-etal-2023-divide} has tried to use a mixture of semantic-independent experts to solve zero-shot DST. It divides dialogues into different clusters based on the dialogue contexts, trains a semantic-independent expert for each cluster, and fuses the parameters of all experts to do an ensemble inference, which surpasses the model with just one expert in all domains.

With the rapid development of large language models (LLM), some studies \citep{NEURIPS2020_1457c0d6,min-etal-2022-rethinking,heck-etal-2023-chatgpt} show that LLM can solve any task without task-specific fine-tuning, but solely with the knowledge they acquired during self-training on massive amounts of data. These LLMs perform well on in-context learning (ICL), where only some natural language prompts and examples are provided to condition the generation process, achieving significant improvements in few-shot learning compared to fine-tuning. \citet{heck-etal-2023-chatgpt} uses ChatGPT as a DST model in the zero-shot experiment and surpasses most of the traditional models in the zero-shot experiment.

% zhutong：第四段：实验结果和优势
%   我们在两个数据集中做了实验
%   相较于小模型提升了多少
%   相较于大模型提升了多少
%   相较于大模型，我们可以节省多少训练代价
%   从聚类结果中，我们发现不同的领域之间存在很多联系
%   相较于所有领域共享同一批prefix prompt，我们发现特异化专家（k>1）对结果有着很好的帮助

In this study, we propose a new method named MPPE-DST which consists of a mixture of deep prefix prompts for LLM's conditional generation. We adopt a large language model to develop its ability of DST. To preserve the ability of the LLM itself, strengthen the robustness of the whole model, and reduce training costs, we freeze the whole parameters of the LLM, add a prefix prompt model to the backbone model and only tune the parameters of the prefix prompt model. The experiment result shows that our MPPE-DST significantly outperforms traditional DST models and does as well as LLMs larger than 100B parameters in zero-shot scenarios.

% zhutong：第五段：总结贡献点
%   针对zero-shot DST中领域知识的迁移问题，我们设计了一种特异化专家方法
%   针对大模型训练代价过高的问题，我们采用Prefix prompt作为不同的专家，用较少的训练代价提升了生成能力
%   我们在两个广泛使用的DST benchmark上进行了测试，并达到了SOTA，结果甚至超过了ChatGPT和fine-tune的100B Codex

Our contributions to this paper are the following aspects:
\begin{itemize}
    \item We utilize deep prefix prompt tuning to improve the ability of the LLM's conditional generation in the DST task.
    \item We propose a novel DST model MPPE-DST which consists of LLM and a mixture of prefix prompt experts.
    % \footnote{Our code is available at \href{https://github.com/ttw1018/MPPE-DST}{github.com/ttw1018/MPPE-DST}} 
    \item Empirical results show that our MPPE-DST works well in zero-shot scenarios and outperforms most of the DST model.
\end{itemize}

==> chapter/result.tex <==
% \input{table/zero-shot-result.tex}
\section{Results \& Analysis}

\subsection{Main Results}

\paragraph{Results on MultiWOZ2.1} Table~\ref{table:zero-shot-result} shows the results of our proposed model on MultiWOZ2.1 under zero-shot setting. We find that our MPPE-DST outperforms all compared baselines on average JGA, achieving a 0.20\% increase over IC-DST CodeX which is a large language model over 100B parameters. Compared to those DST models smaller than 10B parameters, our MPPE-DST achieves over 20\% increase on average JGA. However, we find the performance of the hotel domain is significantly lower than the other 4 domains. We suspect that because it has many unique slots, which share few similarities and correlations with other domains (i.e. ``hotel parking'', ``hotel stay'').

\paragraph{Results on SGD} Table~\ref{table: sgd-result} shows the results of our proposed model on SGD. Our MPPE-DST outperforms all compared baselines greatly with an increase of more than 15\% on average. We find that our MPPE-DST works best on ``Alarm'' because the slots of ``Alarm'' are ``Alarm name'' and ``Alarm time'' and there are many slots associated with ``name'' and ``time'' in other domains.

==> fig/cluster-example.tex <==
\begin{figure*}
    \centering
    \begin{minipage}{.48\textwidth}
        \includegraphics[width=\textwidth]{img/embedding-cluster-example.pdf}
    \end{minipage}
    \begin{minipage}{.48\textwidth}
        \includegraphics[width=\textwidth]{img/hidden-cluster-example.pdf}
    \end{minipage}
    \caption{The visualization of the clustering result. The left is the clustering result of word embedding and the right is the clustering result of hidden output.}
    \label{fig: cluster example}
\end{figure*}

==> fig/heatmap.tex <==
\begin{figure}
    \centering
    % \begin{minipage}{.4\textwidth}
    \includegraphics[width=.48\textwidth]{./img/heatmap-all.pdf}
    % \centering
    % \caption{Cosine similarity for all slots.}
    % \end{minipage}
    % \begin{minipage}{.4\textwidth}
    %     \includegraphics[width=\textwidth]{./img/heatmap-clustering.pdf}
    %     \centering
    %     % \caption{Cosine similarity for slots in the same subset.}
    % \end{minipage}
    % \caption{Cosine similarity visualization. The rows and columns are the slots in MultiWOZ2.1. The image is the cosine similarity visualization of MPPE with 1 cluster and the right image is the cosine similarity visualization of MPPE with 5 clusters.}
    \caption{Cosine similarity visualization. The rows and columns are the slots in MultiWOZ2.1 excluding the restaurant domain.}
    \label{fig: heatmap}
\end{figure}


==> fig/num-clusters.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.48\textwidth]{./img/num-clusters.pdf}
    \caption{The results of different numbers of clusters under zero-shot experiments.}
    \label{fig: number-cluster}
\end{figure}

==> table/mppe.tex <==
\begin{table}
    \centering
    \begin{tabular}{ccc}
        \toprule
        model        & JGA \\
        model + ICL  & ??  \\
        model + DPPT & ??  \\
        \bottomrule
    \end{tabular}
\end{table}
